Your Large Language Models Are Leaving Fingerprints

It has been shown that finetuned transformers and other supervised detectors effectively distinguish between human and machine-generated text in some situations arXiv:2305.13242, but we find that even simple classifiers on top of n-gram and part-of-speech features can achieve very robust performance on both in- and out-of-domain data. To understand how this is possible, we analyze machine-generated output text in five datasets, finding that LLMs possess unique fingerprints that manifest as slight differences in the frequency of certain lexical and morphosyntactic features. We show how to visualize such fingerprints, describe how they can be used to detect machine-generated text and find that they are even robust across textual domains. We find that fingerprints are often persistent across models in the same model family (e.g. llama-13b vs. llama-65b) and that models fine-tuned for chat are easier to detect than standard language models, indicating that LLM fingerprints may be directly induced by the training data.

==> figures/confusion_matrices.tex <==
\begin{figure*}
\centering
\begin{subfigure}{.4\linewidth}
  \centering
  \includegraphics[width=.8\linewidth]{figures/ghostbuster_gpt_claude_cm.png}
  % \caption{Multiclass classification on the Ghostbuster dataset. Our GradientBoost baseline can easily disambiguate between samples written by humans (class 1), ChatGPT (class 2) and Claude (class 3). }
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.4\linewidth}
  \centering
  \includegraphics[width=.8\linewidth]{figures/outfox_chatgpt_flan_cm.png}
  % \caption{Multiclass classification on the Outfox dataset. Our GradientBoost baseline can easily disambiguate between samples written by humans (class 1), ChatGPT (class 2) and Claude (class 3). }
  \label{fig:sub2}
\end{subfigure}
\caption{\textbf{The predictive power of fingerprints.} We show that fingerprints are sufficient not only to separate 'human' from 'machine', but to perform accuracy multi-class classification, distinguishing between texts produced by different models with the same prompt. Here we show multi-class classification results on the Ghostbuster dataset, which includes samples written by humans (class 1), ChatGPT (class 0) and Claude (class 3), and the Outfox dataset, which includes samples written by humans (class 1), ChatGPT(class 0), and Flan (class 2).}
\label{fig:test}
\end{figure*}

==> sections/2_fingerprints.tex <==
\section*{LLM Fingerprints}

% \yoshi{This is part of the proposed method. This subsection should be under ``Methods'' or a fancy-name section such as ``LLM Fingerprints Removal'', which describes the proposed framework (to be clear, detailed settings such as what models were used should be described in the Evaluation/Experiments section.)}

% Before we explain our fine-tuning, we need to explain in more depth what we mean by fingerprints -- a linguistic style that, in the aggregate, is different from that of humans. And this is different from classic authorship identification!
% have a figure showing an example distribution of POS distribution in human vs machine. 
We find that an inspection of several publicly available machine-generated text detection datasets reveals that, both within-domain and across-domain, there are differences in the distribution of lexical and morphosyntactic features between human and machine provenance (\autoref{fig:radial_fingerprints}). 

\citet{li_deepfake_2023} conduct linguistic analysis on their corpus, DeepfakeTextDetect, and find insignificant differences across POS-tag distributions between human and machine data when considering all models and domains in aggregate; however, these distributions begin to diverge when only considering a subset of models or domains.   

\citet{hc3} also notice and comment upon the differences in POS-tag distribution between their collected ChatGPT and human data, positing that this discrepancy may be the result of the RLHF process. 

We conduct linguistic analysis of the same data on a more granular basis, comparing linguistic distributions across and within model families, finding that distinct patterns emerge. The distribution of models within the same family are more similar to each other than to models of other families.

% This pattern implies that the be from the RLHF process, as these models were not fine-tuned before generating this data, as \citet{hc3} posits, and we show that these differences, while slight, are enough of a signal to train a highly accurate n-gram feature based classifier. 
% [Deepfake and HC3, and OpenAI] have also noted this phenomenon.\cite{}
% These distributional differences appear at the token level, and so reveal a surprising intuition that a classifier which makes use of token-level data should perform well on this data. We report the results of such experiments in \autoref{sec:results}.
% \input{tables/authorship}
% Here we substantiate more
\begin{itemize}
    \item  In an experiment of evaluating a GB classifier on two different testsets, one from a different domain with text produced by the same model vs one from the same text domain produced by a different model, there is an appreciable difference in machine class recall. \textbf{In other words, it is easier to detect text produce by the same model in a different domain, than by a different model in the same domain.}
    \item Parallel datasets give us a chance to perform multiclass classification, and we find that chatgpt and flan from outfox, as well as gpt and claude from Ghostbuster, can be easily disambiguated. In contrast, multi-class experiments involving models from the same model family don't work as well.

\end{itemize}
% 

In this work, we use the term ``LLM fingerprint,'' to encompass the idea of a distinctive set of linguistic characteristics that, in the aggregate, differentiate machine-generated text from human-authored content. This fingerprint may be discerned through variations in parts-of-speech (POS) tag distribution, top token frequency, and dependency structures. 

% this is different from just human author identification. Why? People have theorized that humans have individual grammars, 


We argue that the best test for an AI text detector is being evaluated on text that shows minimal distributional discrepancy to human-authored texts; in other words, has a minimal fingerprint. \autoref{sec:experiments} describes our proposed experimental setup to remove fingerprints, and \autoref{sec:discussion} investigates the efficacy of our approach by examining the performance drop of existing detectors against text generated by our fingerprint-removed model.

==> sections/3_data.tex <==
\section{Data}
% how we actually used the data (all of it)
We use publicly available machine-generated text detection datasets for fingerprint analysis as well as training data for supervised sequence classifiers and a reinforcement learning with human feedback setup.

%% how we preprocessed the data.
Our main experiments use two publicly available machine-generated text detection datasets: OUTFOX \cite{outfox} and DeepfakeTextDetect \cite{li_deepfake_2023}, which we refer to as ``Outfox'' and ``Deepfake'' in this work, respectively.

\citet{Verma2023GhostbusterDT} provide three new datasets for evaluating AI-generated text detection in creative writing, news, and student essays. Using prompts scraped from the subreddit \texttt{r/WritingPrompts}, the Reuters 50-50 authorship identification dataset, and student essays from the online source IvyPanda, they obtained ChatGPT- and Claude-generated responses and made efforts to maintain consistency in length with human-authored content in each domain.

We also analyze data from the Human Comparison Corpus (HC3) \cite{hc3}, which includes questions from publicly available datasets and wiki sources with human- and ChatGPT-generated responses based on instructions and additional context. The resulting corpus comprises 24,322 English and 12,853 Chinese questions, of which we only use the English split.
%
\subsection{Outfox}

Outfox is a parallel human-machine dataset built on the Kaggle Feedback Prize dataset \cite{feedback-prize-effectiveness} and contains approximately 15,000 essay problem statements and human-written essays, ranging in provenance from 6th to 12th grade native-speaking students in the United States. For each problem statement, there is also an essay generated by each of three LLMs: ChatGPT (gpt-3.5-turbo-0613), GPT-3.5 (text-davinci-003), and Flan (FLAN-T5-XXL). Each example contain an instruction prompt (``Given the following problem statement, please write an essay in 320 words with a clear opinion.''), a problem statement (``Explain the benefits of participating in extracurricular activities and how they can help students succeed in both school and life. Use personal experiences and examples to support your argument.''), the text of the essay, and a binary label for human or machine authorship.


\subsection{Deepfake}
The Deepfake corpus is a comprehensive dataset designed for benchmarking machine-generated content detection in real-world scenarios \cite{li_deepfake_2023}. It contains approximately 9,000 human examples across 10 text domains, each paired with machine outputs from 27 models (e.g. GPT-3.5-turbo, text-davinci-002) from 7 different model families (e.g. OpenAI), producing several testbeds designed for examining a detector's sensitivity to model provenance and text domain. Each example contains the text, binary label denoting human or machine, and the source information -- which domain, model, and prompting method were used.  
 

% We choose these data splits because they let us examine different questions: 
% This gives us three setups for testing: parallel data produced by one model for one domain (x10), data produced by models within the same family on a number of different domains mixed together, and a parallel set of data in one domain (essay) for three different models. 
% why do we have the outfox data? it's the same prompts from different models, gives us a good comparison across models in just one domain. the multiple single domain single model sets help us to determine the generalizability of the method we propose and the mixed domain helps us identify how strongly correlated to model families the fingerprints are. 

% Together, these different data splits help us to identify fingerprints across models and model families, to determine  
% the domain-specific model-specific testbed data released by [Deepfake]. This data comprises ten distinct sources, each of which may be considered an independent text domain. 

% They use three different prompting methods , continuation 
% This data was originally created by feeding the first 30 tokens (as split by whitespace) of a human text sample to EleutherAI's gpt-j-6b model [deepfake]. Each example in the data comprises the 30-token prompt followed either by the original human response or a machine-generated response. For many of the splits, there is exactly one human-generated response and machine-generated response for each prompt, meaning that the datasets are balanced; however, for some domains, especially those pulled from online forums, there may be many human responses given in response to the same initial prompt, or there may be many machine-generated responses to the same prompt. 


\subsection{Corpus Analysis}
We additionally conduct fingerprint analysis on two other publicly released corpora for supervised machine-generated text detection:
\cite{Verma2023GhostbusterDT} provides three new datasets for evaluating AI-generated text detection in creative writing, news, and student essays. Using prompts scraped from the subreddit r/WritingPrompts, the Reuters 50-50 authorship identification dataset, and student essays from the online source IvyPanda, they obtained ChatGPT- and Claude-generated responses and made efforts to maintain consistency in length with human-authored content in each domain.

We also analyze data from the Human Comparison Corpus (HC3) \cite{hc3}, which includes questions from publicly available datasets and wiki sources with human- and ChatGPT-generated responses based on instructions and additional context. The resulting corpus comprises 24,322 English and 12,853 Chinese questions, of which we only use the English split.

A summary of all datasets used, including their domain coverage and underlying base model(s), may be seen in \autoref{tab:data_splits}.


% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/pos_dist_ex.png}
%     \caption{To be replaced by radial/more analysis plots}
%     \label{fig:dist_diff}
% \end{figure}


% \subsection{Preprocessing}
% Our main pipeline consists of two stages: a supervised fine-tuning (SFT) stage and an RLHF stage. The input data is processed slightly differently for each stage, according to the best practices for each training paradigm. Specifically, we use Direct Preference Optimization (DPO) as our RLHF method. 

% \textbf{SFT:}
% As per the approach suggested by \href{https://arxiv.org/abs/2305.18290}{Rafailov et al. (2023)}, only the positive (i.e., human-generated) texts were used in the SFT process in order to ensure that the model aligns with the data distribution. As such, we filter out all machine-generated responses, leaving us with a training set of approximately half the full number of examples reported in \autoref{tab:data_splits}. 

% Additionally, all of our SFT experiments use a generic, all-purpose instruction prompt: ``Continue the following text: ''. While efforts of prompt-tuning have been shown to improve downstream performance on various tasks [cite], here we leave a thorough exploration of prompt design for future work.

% \textbf{DPO:}
% Direct Preference Optimization requires that the inputs to the model be structured as a triplet of the shared prompt, the chosen tokens, and the rejected tokens. 
% In [Rafailov]'s original setup, both the chosen and rejected responses are generated by an LLM, with the chosen response being the one that a reward model more highly favoured. 
% In our setup, we use the human-generated response as the ``chosen'' input and the machine-generated response as the ``rejected'' input. 

% We truncate the inputs as needed to fit inside the base model's context window and opt to use a training batch size of 1 to use as much context as possible with the same amount of GPU memory.

==> sections/4_models.tex <==
\section{Models}
Models are used mainly for two distinct uses in our paper: generating text and predicting if some text is human or machine-generated. This section describes the models used for each purpose.
\subsection{Natural Language Generation}
% We use a number of large language models of different sizes 
We use 3 recent LLMs as the base models in our experiments: LLaMA-2-7B, and LLaMA-2-13B, and Falcon-7B. We use these models to generate text before and after attempting to remove their fingerprint signatures (through SFT and DPO).
We report training hyperparameter settings and training metrics in \Cref{sec:llm_hyperparams}.
% for classifiers, we use a range, including simple machine learning classifiers, transformer-based classifiers, and the base model + LoRA (sequence classification)


\subsection{Machine-Generated Text Detection}
Like previous work, we use multiple types classifiers to evaluate our methods: feature-based, transformer-based sequence classifier, and zero-shot detection. Unlike \citet{hc3} and \citet{li_deepfake_2023}, we do not use GLTR \cite{Gehrmann2019GLTRSD} features for our feature-based classifier; rather, we use a combination of word, character, and POS n-grams. We limit each of these feature groups to 2000 features. 

We use Longformer  \cite{longformer} for the transformer-based classifier as the input sequences. Some previous work has found finetuned RoBERTa \cite{roberta} models to be effective classifiers; we, like \citet{li_deepfake_2023} instead opt for a model with a larger context window to minimize data truncation. We add a classification head to Longformer and train it for a maximum of 10,000 steps, periodically evaluating on a validation set to monitor overfitting.

Finally, we use DetectGPT for our zero-shot detection method \cite{mitchell_detectgpt_2023}. Following best practices from the original implemenation, we use t3-3b as the paraphrase model and GPTJ-6B as the scoring model. 
% Classifiers we use are taken from the literature Longformer, DetectGPT with GPTj-6B as the detector model, and ours, GB with word, char, and POS features. 

==> sections/8_background.tex <==
\section{Related Work}
% \yoshi{Unless discussing some papers before introducing the proposed method is crucial, I generally put Related Work section right before Conclusion. Also, in the current framing, the connection b/w ``Author Identification'' and ``Machine-generated text detection'' is not clear.}

% \yoshi{Watermarking methods should be mentioned and why we do not consider the approach (i.e., out of the scope of the paper) should be explicitly described. We should clarify the relationship b/w watermarking and fingerprints as well. For example, LLM fingerprints are different from LLM watermarking in the sense that they are inherently acquired during the pre-training process while watermarking is intentionally implemented by the developer.}
% Authorship verification/stylometric analysis
\subsection{Author Identification}
% The underlying premise of author identification is that an author imprints her work with a characteristic writing style. Mark Twain used colloquial dialects, Cicero relied on rhetoric. If we can quantify the ineffable sense of authorial ``voice``, we have a feature set for distinguishing whether a given piece of work was likely penned by a certain author. Historically, a combination of linguistic features 
% a translation of semantic information to geometric space
The origin of modern computational methods for identifying the author of a given text can be traced back to a pivotal study of the Federalist papers conducted by \citet{mosteller_inference_1963}.
This seminal work, conducted in the mid-20th century, utilized stylometric features to discern the authorship of these historical documents. 
Stylometry, an approach analyzing linguistic style and patterns, became a cornerstone in the field of authorship attribution [stomatos, koppel, many others].
Subsequent advances in machine learning, natural language processing, and statistical modelling have propelled the evolution of authorship attribution methods, with more recent work focused on using neural embedding methods to build an authorship representation [cite BertAA and many others]. 

Many formulations of the same base task exist, including predicting the author from a closed set of known authors (author attribution), predicting whether two pieces of text were written by the same author (author verification), or identifying if and where the author changes within a given piece of text (style change detection) [cite PAN].
The realms of application for such computational methods range widely from identifying author changes in ancient historical texts [koppel] to linking anonymous digital communications on the dark web [cite Nick's work, Alice Hutchins] to being utilized in forensic investigations [cite Cristina/Alice Hutchins/Andrew].

% Existing  methods and how we're different
\subsection{Detecting Machine-Generated Text}
Machine-generated text-detection represents a contemporary evolution of traditional authorship identification tasks, specifically directed at discerning whether a given text originates from a language model or a human author. 
Various approaches have been devised to address this novel challenge, although authorship identification methods have not often been applied directly to machine-generated task-detection..
It has been reported that human annotators perform only slightly better than random at this task \cite{clark_all_2021}, although, with training, that number may be improved [cite]. 
Regardless, there is much desire for robust automatic classification method.


While $n$-gram frequencies have often been used for author identification (cite koppel and stomatos? here), only a few recent works have examined the use of hand-crafted features or stylometrics in machine-generated text detection (japenese stylometrics). 
One example is GLTR: a unique system that uses the top-k words to visually highlight text spans likely to be generated by an LLM [cite GLTR].
GLTR is not a detector itself, per se, as its aim is to visually aid humans in the task of spotting AI-written text themselves.


One more common approach to machine-generated text detection is to train a supervised binary classifier on labelled data. [OpenAI] released a detector that was a GPT model fine-tuned in this manner; however, it required an input text length of at least 1,000 characters and was eventually retired due to poor performance [cite that news release]. 
[Deepfake] proposed a variety of classification testbeds, methodically mixing data generated by 27 different models in a number of domains to rigorously test the ability of supervised classifiers to generalise to unseen domains and unseen models, finding that pre-trained language models performed the best, but still a  suffered significant performance drop on out-of-distribution data. 
[Ghostbuster] proposes using a series of weaker language models, including $n$-gram models to determine features on which to train an ensemble classifier. 
The downside of this approach, in particular, is that it requires access to multiple language models for inference, which may be resource- or cost-prohibitive.
% other work has taken a white-box approach -- requiring access to a model's 


Other work has used a zero-shot classification approach, relying, rather than on labelled data, on a model's prediction distribution of an input sequence to make its classification. 
To this end, [DetectGPT] relies on differences in the negative curvature regions of the model's log probability to classify test, while GPTZero relies on thresholding a mixture of perplexity calculations and  `burstiness'. 
These so-called "white box" methods assume access to the underlying LLM for probability estimations, which is not always available for off-the-shelf methods.
Furthermore, white-box methods are known to be susceptible to adversarial attacks. 
Minute changes to a given sequence can heavily affect its perplexity, and even the inclusion of a single space can drastically affect the performance of detectors, as [evade detection via a single space] shows. 

% Watermarking
[cite watermarking] propose adding a ``watermark'' to LLMs in order to render their outputs more detectable. 

% How other people have tried to make more robust classifiers
\subsection{Adversarial Methods}

A variety of adversarial attacks have proved effective against AI-text detectors [cite some].
Recognizing the shortcomings of existing detection methods, some have proposed creating more robust classifiers by augmenting training corpora with more challenging examples.
Recently, [Outfox] proposed using perturbed (e.g. paraphrased) text to augment training data.
While this work also aims to generate more challenging data for more robust detection, we accomplish this by using a reinforcement learning fine-tuning method for our model to produce a more human-like output, rather than a traditional adversarial setup.

% It remains an open question whether either white-box or black-box methods are able to reliably generalize to the task for out-of-distribution data, for data generated by families of models, or for short input sequences. 


==> sections/results_cut_by_rich.tex <==

% what we actually saw happen
\textbf{Fingerprints are often consistent within a model family}
% We visualize fingerprints by looking at the difference of distribution in various linguistic properties. In \autoref{fig:radial_fingerprints}, we report part-of-speech tag distributions of data generated by different models on the same deepfake data domains\footnote{We choose to report POS results in the main paper as it directly maps to one feature set for our classification experiments whereas we do not directly use named entity categories, dependency classes, or top-$k$ words as features.}.  
% Here's where we put a table of or just write a jensen shannon difference for NE, Const, and Top-k for each model family (average +/- std) -- averaged over individual models.
In the \autoref{sec:appendix} we also include analysis from named entity tags, constituency types, and top-\textit{k} most frequent tokens. The strength of the fingerprint is more evident across some axes than others, and there are, of course, more dimensions of linguistic analysis that could theoretically be applied to uncover model fingerprints.

Distinct patterns emerge when comparing the fingerprint of models within the same family compared to models of different families. The degree of similarity within families can vary between families; for example, LLaMA models exhibit a particularly uniform fingerprint across model sizes, while BigScience models (cf. \autoref{sec:appendix}) look markedly different. We believe that part of the imprinting process for models comes from the underlying distribution of training data, so it is possible that differences in training data have a large influence on the visualizations presented here. We leave for future work further analysis of the effect dataset collection, pre-processing, and training objective have on imparting a model's fingerprint.

% As we use linguistic features, we can think of this a
% predictive power of features as indicative of the strength of the fingerprint. 

% here we also talk about how it is analagous
A particularly interesting finding is that our classifier is better at detecting out-of-domain texts from the same model than it is detecting in-domain texts from a different model. In other words, Flan T5 ``sounds'' like T5 whether it is generating news stories or fan fiction.  In \autoref{fig:ood_v_oom} we report the results of taking a classifier trained on data from one model and looking at a drop in machine recall when evaluated on either an in-domain test from from a different model or an out-of-domain test from the same model. The classifier is far more effective in the latter case, and the 95\% confidence interval computed with bootstrapping tells us that this is not due to particular oddities of the data splits we used, but that is it a meaningful result. 

We also explicitly test how well a classifier trained on one model generalizes to (1) other models in the same family and (2) other model families. We find that, on average, the drop in machine recall value (out of 1) from in-domain data to other models in the same family is only 0.04, while the drop to other other families is 0.62. We report these results in \autoref{tab:ood_v_oom}. 

% Taken together, we show that individual LLMs and families of LLMs have unique writing styles which may be captured by the feature sets we propose. 



\textbf{AID methods are generally effective for LLM text detection in publicly available datasets.}
\input{tables/summary_domain_specific}
\input{tables/summary_mixed_domain}



\input{tables/m4}
% it does well in the simple case of binary, one model/one domain
In the most simplistic setup (cf. \autoref{tab:summary_domain_specific}), binary classification of ``human'' or ``machine'' where data is from one model in one text domain, our GradientBoost classifier with linguistic features achieves upwards of 0.94 AUROC on every test. 

% in the case of one model/mixed domains
We also compare the classifier performance on data produced by a single model, but in multiple domains mixed together, seen in \autoref{tab:summary_mixed_domain}. While performance in general is robust, M4's Cohere data is a clear outlier, only achieving 0.64 AUROC, perhaps indicating that it shows a high degree of linguistic diversity across domain-specific generations. However, in a comparison of linguistic vs. neural features on the M4 dataset, we find that the GB classifier can achieve high performance on Cohere (cf. \autoref{tab:summary_m4}).

% in the case of multiclass, one domain
In a multi-class setup (\autoref{tab:multiclass}), where the classifier must distinguish between ``human'', ``model 1'', and ``model 2'', it achieves an average of 0.94 and 0.91 for the Ghostbuster and Outfox datasets, respectively. 

% in the case of mixed model families, it dips
% Finally, we examine the case of LLM content from model families in multiple domains in Deepfake's data. This 

% generalizing to out-of-domain data
All of the above are calculated using unseen data from the same distribution as the training data, but we see strong out-of-domain performance as well in \autoref{fig:deepfake_ood}. Choosing the largest model in each model family available in Deepfake's data, we calculate the F1 score for both an in-domain and out-of-domain test set. Through multiple independent trials and our bootstrapped confidence intervals, we see that F1 on unseen domains has a larger variance, but that overall the difference in F1 score for in-domain and out-of-domain performance is not statistically significant because the confidence intervals overlap. In other words, linguistic features + ML classifiers do generalize well to data in unseen domains.  



% Lowest performance is seen on test sets with generations mixed from multiple models in a binary classification setup, as generations from multiple models essentially muddy the signal from competing fingerprints. However, a classifier trained on a mixed set of models from across families suffers less drop in performance when being evaluated on an unseen model, suggesting that the classifier is able to pick up on general difference between machine and human writing, as well as model-specific fingerprints.

% In general, a GradientBoost classifier trained on only one model or model family does not generalize well to models from another family. On average, a classifier trained on one model family evaluated on another suffers a 0.62 drop in machine recall, 0.21 drop in F1 score, and 0.44 drop in AUC.  

% \textbf{Fingerprints are consistent across datasets.}
% here is where we would look at ChatGPT* and the fingerprints (represented as a jsd table ) for the similar domains. Difficult bc we don't have anything great to compare it to. but oh well. 

% \textbf{Fingerprints hold predictive power across domains; they render more signal across models than they do across domains.}

% Here we talk about figure 2, showing ood vs oom, and figure 4, that there is not a statistically significant drop for out of domain data.

% also grab a superset 

The above results lead us to the surprising conclusion that LLM text detection is analogous to authorship identification. The premise of handcrafted feature-based approaches to authorship identification is that humans have unique, pervasive writing styles that are detectable at the surface level (i.e. word choice, sentence structure). We repeatedly find that the same is true of LLMs. 

\textbf{Robustness to adversarial attacks} 
Included in the Outfox dataset are two adversarially generated test sets on ChatGPT data; one is attacked using DIPPER \cite{krishna2023paraphrasing}, a paraphrase model leveraging paragraph-level context, and OUTFOX \cite{outfox}, a GAN-like method to find effective prompts for adversarial outputs with in-context learning. We evaluate to what extent linguistic and pre-trained neural features are robust to these attacks compared to two baselines: a Longformer \cite{beltagy2020longformer} model fine-tuned on Deepfake data available on the Huggingface Hub \cite{wolf2020huggingfaces}, and an open-source implementation\footnote{\url{https://github.com/BurhanUlTayyab/GPTZero}} of GPTZero \cite{tian2023gptzero}, a zero-shot method for GTD. For every detector, DIPPER is more challenging than OUTFOX. The Deepfake Longformer actually improves on the adversarial sets, although performance is still quite low overall. Linguistic features or BERT features with either a GB classifier or Logistic Regression classifier slightly degrades on DIPPER but is not highly effected by OUTFOX's attacks. 
\autoref{tab:adversarial} 

% \textbf{Fingerprints are semi-domain agnostic: they render more signal across models than they do across domains.}



% We explicitly test how well a classifier trained on one model generalises to (1) other models in the same family and (2) other model families. We find that, on average, the drop in machine recall value from in-domain data to other models in the same family is only 0.04, while the drop to other other families is 0.62. We bootstrap confidence intervals by sampling, with replacement, the recall drop 

% Although the differences of distributions are small in real-terms, they apparently provide enough signal not only for a binary classifier, but for a multi-class classifier to achieve high accuracy when generations from multiple models are combined. We show in \autoref{tab:multiclass} multi-class classification problems on two of our test corpora, Ghostbuster and Outfox. The classifier easily is able to distinguish between Claude, human, and ChatGPT data in one experiment; ChatGPT, human, and Flan in the other. Note that this result may be less strong if the two models were from the same family.

% The above results lead us to the surprising conclusion that LLM text detection is similar to authorship identification. The premise of handcrafted feature-based approaches to authorship identification is that humans have unique, pervasive writing styles that are detectable at the surface level (i.e. word choice, sentence structure). We repeatedly find that the same is true of individual LLMs. 


\textbf{Instruction-tuning manipulates the fingerprint.}

We were curious as to whether instruction-tuning plays a role in substantially increasing or decreasing a model's fingerprint. To test this, we used both the instruction-tuned (`chat') versions of LLaMA-2-7B and LLaMA-2-13B to generate machine responses to human prompts in the deepfake and outfox datasets\footnote{More specifics about generation may be found in the Appendix.}. We then compare fingerprints of the resulting generations, using POS-tag distributions as a proxy. \autoref{fig:chat_vs_base_POS_distrs} illustrates that chat models are more similar to the frequency profile of humans. We also train GB classifiers on our outputs and find that chat models are easier to detect than regular models. We therefore conclude that instruction-tuning increases a model's fingerprint, making it easier to detect with feature-based classifiers. We leave to future work verifying the generalizability of this finding to other models and instruction-tuning regimes.

% then we use both the chat and regular versions of llama to generate responses to outfox and deepfake human prompts and 
% we compare fingerprints by the proxy of POS tag distributions
% chat-13b is easier to detect.

% I don't have time to run that final one

==> tables/classifier_performance.tex <==
\begin{table*}[htbp]
\footnotesize
    \centering
    
    \label{tab:classifier_comparison}
    \begin{tabular}{lcccc|cccc} \toprule
        \multirow{2}{*}{Classifier} & \multicolumn{4}{c}{Original Data} & \multicolumn{4}{c}{Our Data} \\
        \cmidrule(lr){2-5} \cmidrule(lr){6-9}
         & HumanRec & MachineRec & AvgRec & F1 & HumanRec & MachineRec & AvgRec & F1 \\
        \midrule
        Ours &  &  &  &  &  & \\
        GPTZero &  &  &  &  &  & \\
        DetectGPT &  &  &  &  &  & \\
        Ghostbuster &  &  &  &  &  & \\
        \bottomrule
    \end{tabular}
    \caption{Classifier Performance Comparison -- here we want to show that ours suffers a smaller performance drop}
\end{table*}

==> tables/main_results.tex <==
\begin{table*}[h]
\footnotesize
    \centering
    \begin{tabular}{cc|ccc}\toprule
               % &     & Base & \multicolumn{2}{c}{SFT}  & \multicolumn{2}{c}{RLHF} \\ \cmidrule(lr){4-7}
     \textbf{Classifier} & \textbf{Generative Model} & \textbf{Base} & \textbf{SFT}  & \textbf{DPO-same} & \ \midrule
    GradientBoost
            & LLaMA-7b & 1.0 & 0.95 &\round{2}{0.900278940027894}& 0  \\
            & LLaMA-13b & 1.0  & \round{2}{0.9093333333333333} & \round{2}{0.94947209653092}    \\
            & Falcon-7b & xx.xx & xx.xx & xx.xx   \\
            \midrule
    % Longformer 
    %         & LLaMA-7b &xx.xx & xx.xx & xx.xx& xx.xx \\
    %         & LLaMA-13b & xx.xx & xx.xx& xx.xx & xx.xx \\
    %         & Falcon-7b & xx.xx & xx.xx & xx.xx & xx.xx  \\ \midrule
DetectGPT 
            & LLaMA-7b & xx.xx & xx.xx & xx.xx  \\
            & LLaMA-13b & xx.xx & xx.xx & xx.xx  \\
            & Falcon-7b & xx.xx & xx.xx & xx.xx  \\
            \bottomrule
    \end{tabular}
    % mention that a random classifier would give 0.50. Depending on how far away we are, we see that we have a ways to go
    \caption{in-domain (outfox)}
    \label{tab:main_results}
\end{table*}

\begin{table*}[h]
\footnotesize
    \centering
    \begin{tabular}{cc|cccc}\toprule
               % &     & Base & \multicolumn{2}{c}{SFT}  & \multicolumn{2}{c}{RLHF} \\ \cmidrule(lr){4-7}
     \textbf{Classifier} & \textbf{Generative Model} & \textbf{Base} & \textbf{SFT}  & \textbf{DPO-same} & \textbf{DPO-random}\\ \midrule
    GradientBoost
            & LLaMA-7b & \round{2}{0.9473684210526315} & \round{2}{0.1232} &xx.xx& xx.xx  \\
            & LLaMA-13b & \round{2}{0.8512396694214877}  & \round{2}{0.3656} & xx.xx & xx.xx   \\
            & Falcon-7b & xx.xx & xx.xx & xx.xx & xx.xx  \\
            \midrule
    % Longformer 
    %         & LLaMA-7b &xx.xx & xx.xx & xx.xx& xx.xx \\
    %         & LLaMA-13b & xx.xx & xx.xx& xx.xx & xx.xx \\
    %         & Falcon-7b & xx.xx & xx.xx & xx.xx & xx.xx  \\ \midrule
DetectGPT 
            & LLaMA-7b & xx.xx &  xx.xx &  xx.xx & xx.xx \\
            & LLaMA-13b & xx.xx &  xx.xx &  xx.xx & xx.xx \\
            & Falcon-7b & xx.xx &  xx.xx & xx.xx & xx.xx \\
            \bottomrule
    \end{tabular}
    % mention that a random classifier would give 0. Depending on how far away we are, we see that we have a ways to go
    \caption{out-of-domain (deepfake)}
    \label{tab:main_results}
\end{table*}

